On Packing Low-Diameter Spanning Trees

Edge connectivity of a graph is one of the most fundamental graph-theoretic concepts. The celebrated tree packing theorem of Tutte and Nash-Williams from 1961 states that every $k$-edge connected graph $G$ contains a collection $\cal{T}$ of $\lfloor k/2 \rfloor$ edge-disjoint spanning trees, that we refer to as a tree packing; the diameter of the tree packing $\cal{T}$ is the largest diameter of any tree in $\cal{T}$. A desirable property of a tree packing, that is both sufficient and necessary for leveraging the high connectivity of a graph in distributed communication, is that its diameter is low. Yet, despite extensive research in this area, it is still unclear how to compute a tree packing, whose diameter is sublinear in $|V(G)|$, in a low-diameter graph $G$, or alternatively how to show that such a packing does not exist. In this paper we provide first non-trivial upper and lower bounds on the diameter of tree packing. First, we show that, for every $k$-edge connected $n$-vertex graph $G$ of diameter $D$, there is a tree packing $\cal{T}$ of size $\Omega(k)$, diameter $O((101k\log n)^D)$, that causes edge-congestion at most $2$. Second, we show that for every $k$-edge connected $n$-vertex graph $G$ of diameter $D$, the diameter of $G[p]$ is $O(k^{D(D+1)/2})$ with high probability, where $G[p]$ is obtained by sampling each edge of $G$ independently with probability $p=\Theta(\log n/k)$. This provides a packing of $\Omega(k/\log n)$ edge-disjoint trees of diameter at most $O(k^{(D(D+1)/2)})$ each. We then prove that these two results are nearly tight. Lastly, we show that if every pair of vertices in a graph has $k$ edge-disjoint paths of length at most $D$ connecting them, then there is a tree packing of size $k$, diameter $O(D\log n)$, causing edge-congestion $O(\log n)$. We also provide several applications of low-diameter tree packing in distributed computation.

==> dist-app-short.tex <==
Our improved distributed algorithms in highly-connected graphs are based on the following basic tool, which follows by combining Karger's edge sampling and the diameter-fixing Theorem \ref{thm:random_tree_planting}.
\begin{claim}[Basic Distributed Tool]\label{cl:basic-dist-tool-main}
There is a randomized algorithm that, given a $k$-edge connected $n$-vertex graph $G$ and a congestion bound $\eta \in [1,k]$, computes,  in $\widetilde{O}((101k\ln n/\eta)^{D})$ rounds, a collection of $k$ spanning trees that cause total edge-congestion at most $O(\eta\cdot\log n)$, and have diameter at most $O((101k\ln n/\eta)^{D})$ each. 
Moreover, the algorithm can compute $k$ spanning subgraphs with similar congestion and diameter bounds in $O(D+\eta\log n)$ rounds. The round complexity, the diameter, and the congestion bounds hold with high probability.
\end{claim}
%Throughout in this section, we consider graphs with constant diameter, i.e., $D=O(1)$.  \mynote{JC: is this right? Thm 21 is stated for higher values of $D$}

\paragraph{Approximation of Minimum-Cut.} Ghaffari and Kuhn \cite{ghaffari2013distributed,GhaffariThesis17} gave a very simple approach for finding an $O(\log n)$-approximation for the minimum cut problem that is based on Karger's edge sampling technique. The round complexity of their algorithm is $O(\sqrt{n})$ for constant diameter graphs. Combining Theorem \ref{thm:Karger_diameter} with Ghaffari and Kuhn's algorithm immediately leads to an $\widetilde{O}(\lambda)$ algorithm for graphs with constant diameter, where $\lambda$ is the size of the minimum-cut. 

To provide a more general approach for improved algorithms in highly-connected graphs, we next describe the notion of low-congestion shortcuts.
 %improved shortcuts for highly connected graphs of small diameter. The latter allows us to provide improved algorithms in highly connected graphs for several graph problems (e.g., MST).  \mynote{JC: Is this result now obsolete due to the Ghaffari et al work? Should it be taken out?}

\paragraph{Low-Congestion Shortcuts.} This notion, introduced by Ghaffari and Haeupler \cite{GhaffariH16}, provides a modular framework for solving global graph problems in the distributed setting.
\begin{definition}[Low-Congestion Shortcuts, \cite{GhaffariH16}]
Given a graph $G=(V,E)$, and a partition  $S_1,\ldots, S_N$ of $V$ into disjoint subsets, such that for all $1\leq i\leq N$, graph $G[S_i]$ is connected, an $(\alpha,\beta)$-shortcut is a collection $\{H_1,\ldots, H_N\}$ of subgraphs of $G$,  that  satisfy the following: 
\begin{itemize}
\item{(1)} for each edge $e \in E$, there are at most $\alpha$ subgraphs $G[S_i]\cup H_i$ containing $e$; and
\item{(2)} the diameter of each subgraph $G[S_i]\cup H_i$ is at most $\beta$.
\end{itemize}
\end{definition}
Ghaffari and Haeupler \cite{GhaffariH16} showed that the quality of algorithms for several basic problems depend on the sum of $\alpha$ (i.e., congestion) and $\beta$ (i.e., the dilation). The quantity of $\alpha+\beta$ is usually referred to as the \emph{quality} of the shortcuts.
As observed by \cite{GhaffariH16} for every $n$-vertex graph $G$ and any collection of vertex-disjoint subsets $S_1,\ldots, S_N$, there exist $(\alpha,\beta)$ shortcuts for with $\alpha+\beta=O(D+\sqrt{n})$. 
Our key result is in providing a nearly optimal construction for low-congestion shortcuts in highly connected graphs of constant diameter.
\begin{theorem}\label{lem:dist-shortcuts-construction}[Improved Shortcuts in Highly Connected Graphs]
There is a randomized algorithm that, 
for a sufficiently large $n$, given any $k$-connected $n$-vertex graph $G$ of diameter $D=O(\log n/\log\log n)$, together with a partition $\{S_1,\ldots, S_N\}$ of $V(G)$, such that for all $1\leq i\leq N$, $G[V_i]$ is a connected graph, w.h.p. computes $(\alpha,\beta)$ shortcuts, with $$\alpha+\beta=\widetilde{O}(\min\{\sqrt{n/k}+n^{D/(2D+1)}\},n/k),$$
in $\widetilde{O}(\alpha+\beta)$ rounds. %Both the round complexity and the correctness hold with high probability.
\end{theorem}
%
%\mynote{JC: it's not good to say that correctness holds with high probability. Instead w.h.p. should be put into the thm body where appropriate e.g. "w.h.p. computes $(\alpha,\beta)$ shortcuts in x rounds".}

The construction of the shortcuts from Theorem \ref{lem:dist-shortcuts-construction} serves the basis for the proof of Theorem \ref{thm:mstdist}. In the full version of the paper we describe further algorithmic applications of our results for additional graph problems. The proof of Theorem \ref{lem:dist-inf-diss} is  based on a careful implementation of Claim \ref{cl:basic-dist-tool-main}.

